Resolution-of-identity approach to Hartree-Fock, hybrid density functionals, RPA, MP2, and \textit{GW} with numeric atom-centered orbital basis functions

Efficient implementations of electronic structure methods are essential for first-principles modeling of molecules and solids. We here present a particularly efficient common framework for methods beyond semilocal density-functional theory, including Hartree-Fock (HF), hybrid density functionals, random-phase approximation (RPA), second-order M{\o}ller-Plesset perturbation theory (MP2), and the $GW$ method. This computational framework allows us to use compact and accurate numeric atom-centered orbitals (popular in many implementations of semilocal density-functional theory) as basis functions. The essence of our framework is to employ the "resolution of identity (RI)" technique to facilitate the treatment of both the two-electron Coulomb repulsion integrals (required in all these approaches) as well as the linear density-response function (required for RPA and $GW$). This is possible because these quantities can be expressed in terms of products of single-particle basis functions, which can in turn be expanded in a set of auxiliary basis functions (ABFs). The construction of ABFs lies at the heart of the RI technique, and here we propose a simple prescription for constructing the ABFs which can be applied regardless of whether the underlying radial functions have a specific analytical shape (e.g., Gaussian) or are numerically tabulated. We demonstrate the accuracy of our RI implementation for Gaussian and NAO basis functions, as well as the convergence behavior of our NAO basis sets for the above-mentioned methods. Benchmark results are presented for the ionization energies of 50 selected atoms and molecules from the G2 ion test set as obtained with $GW$ and MP2 self-energy methods, and the G2-I atomization energies as well as the S22 molecular interaction energies as obtained with the RPA method.

==> three_center_integral.tex <==
With a prescription to construct ABFs at hand, we need to compute the overlap integrals $C_{ij}^{\mu}$, defined
in (\ref{Eq:SVS_coefficient}) for RI-SVS or in (\ref{Eq:V_coefficient}) for RI-V, respectively. 
We also need their Coulomb matrix given by (\ref{Eq:coulomb_matrix} in general), and in RI-SVS
additionally the ``normal'' overlap matrix $S_{\mu\nu}$ given by (\ref{Eq:ABF_overlap}). 

To reduce the six-dimensional Coulomb integrations to three dimensional ones, we first solve Poisson's Equation for
each $P_\mu(\bfrp)$ (textbook classical electrostatics). We define
$Q_{\mu}(\bfr)$ as 
 \begin{equation}
  Q_{\mu}(\bfr) = \int d{\bfrp} v(\bfr-\bfrp)P_\mu(\bfrp),
  \label{Eq:coulomb_auxil_conv}
 \end{equation}
Using the Laplace expansion of the Coulomb potential $v(\bfr-\bfrp)=1/|{\bf r-r^\prime}|$, 
\begin{equation}
v(\bfr-\bfrp)=\sum_{lm}\frac{4\pi}{2l+1}Y_{lm}(\hat{\bf r})Y^\ast_{lm}(\hat{\bf r^\prime})
\times \frac{r_{<}^l}{r_{<}^{l+1}},
\label{Eq:coulomb_expansion}
\end{equation}
where $r_{<}=\text{min}(r,r')$ and $r_{>}=\text{max}(r,r')$, the
integration of the angular part in (\ref{Eq:coulomb_auxil_conv})
can be done analytically, yielding
 \begin{equation}
  Q_{\mu}(\bfr) = \frac{\alpha_{al\kappa}(r)}{r}Y_{lm}(\hat{\bfr}_a).
 \end{equation}
The radial part $\alpha_{al\kappa}(r)$ is given by a simple one-dimensional 
(numerical) integration \cite{Arfken/Weber:2001,Delley1990,Blum/etal:2009} 
% \begin{widetext}
  \begin{equation}
     \alpha_{al\kappa}(r) = \frac{4\pi}{2l+1} 
    \left[ \left(\int _0^{r} d r_<
\xi_{al\kappa}(r_<) \frac{r_<^{l+1}}{r^{l}}\right) + 
\left(\int _r^{\infty}  d r_>
\xi_{al\kappa}(r_>) \frac{r^{l+1}}{r_>^{l}}\right) \right].
  \end{equation}
% \end{widetext}
Thus, the formally six-dimensional integrals in
(\ref{Eq:coulomb_matrix})  and (\ref{Eq:V_coefficient}) reduce
to three-dimensional ones,
\begin{equation} 
  (ij|\mu) = \int \phi_i(\bfr)\phi_j(\bfr)Q_\mu(\bfr) d\bfr,
 \label{Eq:3center_integral}
\end{equation}
and 
\begin{equation} 
  (\mu|\nu) = \int P_\mu(\bfr)Q_\nu(\bfr) d\bfr.
 \label{Eq:2center_integral}
\end{equation}

({\bf PR: I assume this part has to be adjusted if we include logsbt})
There are numerous ways to perform the resulting two- and three-center
3D integrals in the literature, including, for example, the techniques
developed by Talman,\cite{Talman:2003,Talman:2007} which we are also
actively exploring.\cite{Wieferink/etal:inpreparation} However, the results
in the present work are computed with a simpler technique using
overlapping, atom-centered spherical grids and the same technology
that is used in many quantum-chemical applications for the
exchange-correlation matrix in DFT.\cite{Becke:1988,Delley:1990} The
integration grid points $\bfr=\bfr (a,s,t)$ are uniquely specified by
the atomic center $a$, the radial shell number $s$, and 
angular point $t$. $w(s,t)$ is the corresponding integration
weight. Details of our own implementation (FHI-aims) are given in
\cite{Blum/etal:2009,Havu/etal:2009}. 
Since these are true three-center integrals, we restrict 
the integration domain for a particular integral element to the grids 
associated with the atoms on which the basis functions in  
question are centered.  For instance, denoting the respective atoms by
$a_1$, $a_2$, $a_3$, the three-center integrals  in
(\ref{Eq:3center_integral}) can then be discretized as 
\begin{equation}
   (ij|\mu) = \sum_{a={a_1,a_2,a_3}} \sum_{s,t}p_3(a,\bfr) w(s,t) \phi_i(\bfr)\phi_j(\bfr)Q_\mu(\bfr), 
\end{equation}
where $p_3(a,\bfr)$ is a three-center partition function that satisfies 
\begin{equation}
  \sum_{a=a_1,a_2,a_3}p_3(a,\bfr)=1  \nonumber
\end{equation}
everywhere in the overlapping region of the three functions, and is
zero otherwise. The two-center integrals  (\ref{Eq:2center_integral}) can be
performed in a similar fashion. The underlying numerical grids can in
principle be increased up to arbitrary accuracy if needed.



